An Effective End-User Development Approach Through Domain-Specific Mashups for Research Impact Evaluation

Over the last decade, there has been growing interest in the assessment of the performance of researchers, research groups, universities and even countries. The assessment of productivity is an instrument to select and promote personnel, assign research grants and measure the results of research projects. One particular assessment approach is bibliometrics i.e., the quantitative analysis of scientific publications through citation and content analysis. However, there is little consensus today on how research evaluation should be performed, and it is commonly acknowledged that the quantitative metrics available today are largely unsatisfactory. A number of different scientific data sources available on the Web (e.g., DBLP, Google Scholar) that are used for such analysis purposes. Taking data from these diverse sources, performing the analysis and visualizing results in different ways is not a trivial and straight forward task. Moreover, people involved in such evaluation processes are not always IT experts and hence not capable to crawl data sources, merge them and compute the needed evaluation procedures. The recent emergence of mashup tools has refueled research on end-user development, i.e., on enabling end-users without programming skills to produce their own applications. We believe that the heart of the problem is that it is impractical to design tools that are generic enough to cover a wide range of application domains, powerful enough to enable the specification of non-trivial logic, and simple enough to be actually accessible to non-programmers. This thesis presents a novel approach for an effective end-user development, specifically for non-programmers. That is, we introduce a domain-specific approach to mashups that "speaks the language of users"., i.e., that is aware of the terminology, concepts, rules, and conventions (the domain) the user is comfortable with.

==> chapters/ch9-name-disam.tex <==
% !Tex root = ../phd-thesis.tex

%%% Chapter start. %%%
\chapter{Researchers Name Disambiguation}
\label{chp:namedisam}

\section{Overview}
Research work on the problem of \emph{Name Disambiguation} was not the main focus of this thesis. However, working in the domain of research evaluation, where the name disambiguation problem poses serious challenges for research impact  evaluators, turned us to devise an approach which can effectively solve the very problem. The approach that we present in following is a work-in-progress and its not yet integrated in our mashup platform.
%As a secondary contribution of the thesis, in this chapter we present the problem of \emph{name disambiguation} in the field of research evaluation, especially in the context of \emph{digital libraries} and an approach that we have recently developed. The results that we present in this chapter are based on a work-in-progress, and this feature is not yet integrated in our mashup platform.
 
The \emph{name disambiguation} problem occurs when multiple authors share common name or when multiple name variations of an author appear in citation records. The problem is not trivial to solve and mostly digital libraries do not provide a way to accurately identify the citation records of an author. We propose a heuristic-based, unsupervised method that also involves users’ interaction as to get users’ feedback in disambiguation process. Moreover, the method exploits important features associated with an author and citation records such as co-authors, affiliation, publication title, venue etc. We performed experiments on a set of researchers that are considered highly ambiguous; high precision and recall results of the experiments show the viability of our approach.


\section{Background}
Digital libraries (DLs) such as DBLP, Google Scholar, and Microsoft Academia maintain and provide
bibliographic citation data, thus allow the search and discovery of relevant publications (i.e., citation
records) in a centralized way. To obtain the citation records of an author requires querying a DL with full or
partial name so DL in result returns back a list of citation records that match the given input. The name
disambiguation problem may occur when multiple authors share common name or an author's multiple
name variations appear in DLs due to name abbreviations or misspellings. In both scenarios, it would be
difficult to be certain whether the returned records are correct or not. For example, the full version of an
abbreviated author name "M. Imran" may refer to "Muhammad Imran" or "Malik Imran", two completely
different persons but in DLs both refer as "M. Imran". So when citation records mix up two persons those
having same name variations (e.g., "M. Imran") is known as "mixed citation" [1]. On the other hand, in case
of the exact name search the problem remains, for example, an author name "Muhammad Imran" which is a full name, shared by many other authors having the exact same full name. This problem results in splitting an author's citation records among others whose names are exactly the same. This problem is known as "Split citation" [1].

In the recent years, many attempts have been made to solve the problem. Mainly two kinds of approaches
have been proposed so far: supervised approach [3][4][5][6] and unsupervised approach [1][8][9][10]. The
former requires a set of training data to train a classifier for further disambiguation processing. This process involves tedious human effort, as manual labeling of citation records is not a straightforward task due to many reasons. The latter approach works without training of a classifier that is to consider the author's or citations meta-data. Despite many attempts, both, DLs and the community efforts failed to solve the problem and to provide an adaptive and generic solution that is extendable in behavior.
In this paper we propose a heuristic-based multi-layer real-time unsupervised method. The proposed method exploits both author-specific meta-data features (e.g., author name, co-authors, affiliation etc.) as well as citation-specific meta-data features (e.g., publication title, published venue etc.). The method also considers users’ feedback during the process so to tune subsequent steps for better performance. As our algorithm is based on an unsupervised approach so we do not need to train a classifier hence no need to have a set of correctly manually labeled data to run the disambiguation algorithm. 
%In summary, the main contributions of this work are:

\section{Investigation on Features Selection}
To analyze and accurately assign citation records to their actual researchers, we first investigate on various
associative pieces of information DLs provide along with a citation record. We call these pieces as
"features", and we believe these features, if exploited and used correctly, can be very useful to solve the very problem. We try not to restrict our approach to a particular DL; instead we aim to find a set of common features that almost all DLs share. In this section, we present and elaborate selected common features. Of the selected features, some are directly associated with a researcher and others with a citation record. We use term "citation record", to generally represent various types of scientific resources. For instance, to name a few, these include conference proceedings, journals papers, patents and books etc.

\subsection{Accredited Features}
\subsubsection{Co-Author} 
\emph{Co-author} is defined as a joint author of a book, paper or journal and who has collaborated with others to bring about a particular publication. In this paper, we refer the first author of a citation record as "principal author" and rest of the authors as co-authors. Thus, a co-author instance represents one author among many co-authors other than the principal author. The big advantage of this feature is that it can be easily retrieved from any DL. The heuristic we use with co-author is that, if a co-author appears in two different publications where a same principal author also appears then most likely both publications belong to the principal author that is being investigated. We consider co-author feature as a strong ground truth, unless many other features collectively prove this assumption wrong. As it is less likely that same co-author writes with two different authors (i.e., principal authors) those having exactly the same name.

\subsubsection{Venue}
\emph{Venue} represents an event name that could be a conference, workshop or a journal name where researchers submit their publications. These events organize and target one discipline (i.e., computer science, physics etc.) at a time. And, most of the times an event focus on a very specific sub-discipline within these broad disciplines. For instance, in computer science field a number of such events target only databases community, some other target computer security etc. The advantage of the venue information is that it is a necessary part of a citation record and every DL provides it. The heuristic we make here is that a researcher, throughout his career, tends to publish in some specific sub-disciplines, or some other related fields under one area of science. It is rarely observed that a researcher publishes in cross disciplines, however many researchers change their sub-disciplines but not the general area. So, the venues information of two researchers, having same names, can differentiate one from the other based on examining disciplines and sub-disciplines information of a researcher's interest.

\subsubsection{Affiliation}
\emph{Affiliation} describes the relationship of an author with institute, organization, university where he/she belongs and works for. The affiliation information, when submitting a publication to a conference, journal or a workshop etc., is an obligatory field that must be provided that then served as publication meta-data. Affiliation of an author tends to change with the period of time. To this end, the heuristic we use is an assumption that if two publications with same principal author names, those also share the same affiliation information too so then both publications will be considered as belongs to the same author.

\subsubsection{Name Instances}
\emph{Name Instances} are different name variations that an author can be associated with, which is based on the size of an author name. For instance, "Muhammad Imran", can be written as "M. Imran", "Imran. M", or "Imran Muhammad". As it is evident that many conferences use different name abbreviations sequences of an author, ultimately making confusions for DLs to correctly identify and associate publications to their actual authors. The name variation problem could be even worse when two authors’ shortened name prefix or suffix leads to two completely different names. For instance, "M. Imran" can be "Malik Imran" or "Muhammad Imran" or "Mehmood Imran", which are all true cases. It is important to consider this aspect when performing disambiguation process. In our approach we keep track of these name variations and resolve ambiguities among them at various stages that is described in the next section.

\subsubsection{Title}
\emph{Title} is a string literal, i.e., name of a citation record. Title contains important keywords that can be used for the title similarity check. A list of extracted important keywords from a set of citation records of an author can be help to understand his area of interest thus finding similar interest of other authors who shares same name can actually disambiguate them. We apply this feature at a stage when we firmly confirm about an author's set of citation records.

\subsubsection{Homepage}
\emph{Homepage} is the URL of the author's homepage. If an author has a homepage then it makes disambiguation task easier. We use this feature as a final step so to increase the quality of results.


\section{Disambiguation Using Multilayer Clustering}
\subsection{Approach Overview}
Given the set of selected features we now present how we solve the problem using
unsupervised technique, for that we use hierarchical clustering approach. We form clusters of retrieved
citation records containing both mixed and split records against a user query and disambiguate them. We use DBLP to query the citation records. The process split the data into meaningful sub-clusters according to the heuristics mentioned above. For this purpose we use hierarchical clustering approach, more specifically, we use both the agglomerative and the divisive approaches, where selected features initially form relatively big clusters (i.e., based on divisive approach) and then we split them up recursively as the results of other features whose values fall down to a threshold. Two clusters are merged (i.e., based on agglomerative approach) once the distance between them reduces and reaches to a certain threshold.

To decide which clusters should be combined or split requires measuring similarity as well as dissimilarity
of the features that belong to citation records in a cluster. Within a cluster, we specifically measure the
distance between a pair of features using Levenshtein Distance algorithm [8]. At certain stages, we also
involve users’ feedback on the resultant clusters to get a point to which our algorithm must perform
clustering (i.e., combine, split). To this end, using a web interface we show to user multiple lists of citations records where each list represents a cluster that then the user selects his/her desired list. This helps us to understand the properties of principal cluster (i.e., a cluster that contains citation records of a principal author) that ultimately leads the disambiguation algorithm to a convergence point. We show the overall approach in Figure \ref{fig:name-disam} and in the next section we elaborate each step in detail.


\begin{figure}[t]
  \centering
    \includegraphics[width=\columnwidth]{figs/nameDis-approach-fig.pdf}
  \caption{Name Disambiguation: overall approach}
  \label{fig:name-disam}
\end{figure}

\subsection{Hierarchical Clustering}
As stated above that our approach follows the hierarchical clustering approach that is we divide the whole
process into multiple layers in a sensible way that ultimately produces quality results. Layers are dependent on each other, means we process layers in a sequence; a subsequent layer in the sequence uses the results produced by the previous layer thus improving quality at every step.

\subsubsection{Inter-related disciplines based formation of clusters}
During the first step, which involves the construction of an initial set of clusters, we aim at identifying outliers (i.e., those records that belong to a different discipline than of user’s choice). In this step we build relevantly big clusters that to large extent contains all those inter-related citation records that share a common discipline (e.g., computer science, physics, etc.). To form such clusters, we exploit Venue information of the citation records. It is very intuitive that a cluster after this step must contain all citation records that belong to a common discipline or to a sub-discipline. This means two authors who share common name but work in two different disciplines separated after this step. At the end of this step we present to user the results (i.e., list of clusters) and ask to select his/her desired list. The user intervention at this stage plays an important role as otherwise choosing wrong cluster would never lead algorithm to converge.

\subsubsection{Co-authors based split} 
Once the user’s feedback obtained, we now move to the next step with only one cluster (i.e., user’s selected one). In this step we aim at splitting the selected cluster into sub-clusters (i.e., divisive approach) based on the co-authors feature. We check, for each pair of citation records in the cluster, co-authors similarity measure. If two records share a common co-author then both form a sub-cluster. The
same process recursively checks co-author based similarity for all the records until there is no match found. The result of this step splits the big cluster into a number of sub-clusters. During this step, we also maintain a list of candidate principal authors based on the name variations present in various citation records. So each cluster now has a list of candidate principal authors that we use in the next steps.

\subsubsection{Affiliation based agglomerate} 
At this point, we have a number of clusters and in order to strengthen the credibility of a cluster that whatever it contains is correct, we check affiliation information (i.e., candidate principal authors’ affiliation) across the clusters. We first collect from each sub-cluster the affiliation information, following the publisher URL present in the DBLP data for each record. In some cases, for instance, researcher who works in a university, write in some of their publications the affiliation information as university name and in some other department name also appeared along with the university name. To tackle this problem, as stated above, we use levenshtein distance between two different strings to measure the similarity. We then match affiliation information across clusters to merge closely similar ones that resultantly reduce the number of clusters; hence making them more obvious. To identify correct principal
author, during the merging process we also check the candidate principal authors’ list and replace short
name variation of an author whose match is found in a cluster that is being compared. So at the end of this stage, we only have those clusters that contain citation records having common co-authors’, common
candidate principal authors and common affiliation information; surely consolidate a cluster’s viability. We
now again present to the user the remaining clusters with detail information of citation records, so that the user can select one among them that closely match his choice. As after the user endorsement, the selected cluster will now from this stage on considered principal cluster having principal author and containing the correct information.

\subsubsection{Pursuit of the remaining bits}
Although the previous step gives us fruitful results even then during this step
we strive for the remaining citation records that possibly split among other clusters. To achieve this, we use title and homepage features. In order to check the title similarity, we build a vector representing keywords and their frequencies of all the citation records in a cluster. Prior to build this vector we perform preprocessing steps (e.g., stop-words filtering, stemming etc.). We perform this step for the principal as well as for all other clusters. A similarity measure process runs between the vector of principal cluster and the vectors of all other clusters one by one. If a cluster found with greater similarity then the citation records will be merged in the principal cluster. As a final step, we check for homepage of the principal and the other candidate principal clusters authors. We use Google search API for this purpose. If within first ten organic search results we find principal author name having keyword “homepage” and most of the keywords present in the vectors built during the previous step, then that is considered as the homepage of the author so its URL is maintained. Same process is performed for all other clusters’ authors and we merge those citations records whose homepage URL is same as the principal authors URL. One can note that this feature is powerful, however we do not depend our entire algorithm based on this feature because it appears that many new researchers do not have a homepage.

